A scaled Bregman theorem with applications

Bregman divergences play a central role in the design and analysis of a range of machine learning algorithms. This paper explores the use of Bregman divergences to establish reductions between such algorithms and their analyses. We present a new scaled isodistortion theorem involving Bregman divergences (scaled Bregman theorem for short) which shows that certain "Bregman distortions'" (employing a potentially non-convex generator) may be exactly re-written as a scaled Bregman divergence computed over transformed data. Admissible distortions include geodesic distances on curved manifolds and projections or gauge-normalisation, while admissible data include scalars, vectors and matrices. Our theorem allows one to leverage to the wealth and convenience of Bregman divergences when analysing algorithms relying on the aforementioned Bregman distortions. We illustrate this with three novel applications of our theorem: a reduction from multi-class density ratio to class-probability estimation, a new adaptive projection free yet norm-enforcing dual norm mirror descent algorithm, and a reduction from clustering on flat manifolds to clustering on curved manifolds. Experiments on each of these domains validate the analyses and suggest that the scaled Bregman theorem might be a worthy addition to the popular handful of Bregman divergence properties that have been pervasive in machine learning.

==> src/aditya_scrap.tex <==
%!TEX root = ../bregman-gauge-nips2016.tex

%
\section{Aditya's scrap notes}


%
\subsection{Regret analysis of \citet{kwhTP}}

The proof of \citet{kwhTP} has a few key steps.

\emph{Step 1: Telescoping sum}.
We first note that
$D_{\varphi}(\ve{u}\| \ve{w}_0) = (1/2) \cdot \|\ve{u}\|^2_q$ since $\ve{w}_0 = \ve{0}$, and $D_{\varphi}(\ve{u}\| \ve{w}_{T+1}) \geq 0$, and so
\begin{eqnarray}
(1/2) \cdot \|\ve{u}\|^2_q & \geq & D_{\varphi}(\ve{u}\| \ve{w}_0) - D_{\varphi}(\ve{u}\| \ve{w}_{T+1}) \nonumber\\
  & = & \sum_{t=1}^T  \left\{D_{\varphi}(\ve{u}\| \ve{w}_{t-1}) - D_{\varphi}(\ve{u}\| \ve{w}_{t})\right\}\nonumber \text{ by telescoping property }.
\end{eqnarray}

\emph{Step 2: Bregman triangle equality}.
The Bregman triangle equality brings:
\begin{eqnarray}
\lefteqn{D_{\varphi}\left(\ve{u} \left\| \ve{w}_{t-1}\right.\right) - D_{\varphi}\left(\ve{u} \left\| \ve{w}_{t}\right.\right)} \nonumber \\
& = & \left(\ve{u} - \ve{w}_{t-1}\right)^\top \left(\nabla\varphi\left( \ve{w}_{t}\right)-\nabla\varphi\left( \ve{w}_{t-1}\right)\right) - D_{\varphi}\left(  \ve{w}_{t-1}\left\| \ve{w}_{t}\right.\right) \nonumber\\
 & = & \eta_t \cdot (y_t - \ve{w}_{t-1}^\top \ve{x}_t) \cdot \left(\ve{u} - \ve{w}_{t-1}\right)^\top \ve{x}_t -  D_{\varphi}\left( \ve{w}_{t-1}\left\| \ve{w}_{t}\right.\right) \label{bti2}\:\:,
\end{eqnarray}
where the last line is because $\ve{w}_t = (\nabla\varphi)^{-1}( \nabla\varphi( \ve{w}_{t - 1} ) - \Delta )$ for $\Delta = -\eta_t (\ve{w}_{t-1}^\top \ve{x}_t - y_t) \cdot \ve{x}_t$.
Notice that we implicitly use the fact that $\nabla\varphi \left( \ve{w}_{0}\right) = \ve{0}$ to use Equation (\ref{bti2}) for all $t\geq 1$.

\emph{Step 3: Divergence bound}.
The last divergence term can be bounded by invoking \citet[Appendix I]{kwhTP}, which gives:
\begin{eqnarray}
D_{\varphi}\left(\ve{w}_{t-1} \| \ve{w}_t \right) & \leq & \frac{p-1}{2} \cdot \| \Delta \|_p^2 \\
& = & \frac{p - 1}{2} \cdot \eta_t^2 \cdot (y_t - \ve{w}_{t-1}^\top \ve{x}_t)^2 \cdot \| \ve{x} \|_p^2 \:\:.
\end{eqnarray}
Therefore,
\begin{equation}
	\label{eqn:kivinen-bound}
 	D_{\varphi}\left(\ve{u} \left\| \ve{w}_{t-1}\right.\right) - D_{\varphi}\left(\ve{u} \left\| \ve{w}_{t}\right.\right) \geq \eta_t \cdot (y_t - \ve{w}_{t-1}^\top \ve{x}_t) \cdot \left(\ve{u} - \ve{w}_{t-1}\right)^\top \ve{x}_t - \frac{p - 1}{2} \cdot \eta_t^2 \cdot (y_t - \ve{w}_{t-1}^\top \ve{x}_t)^2 \cdot \| \ve{x} \|_p^2.
\end{equation}

\emph{Step 4: Simplification and choice of $\eta$}.
Let $s_t = \left(\ve{u} - \ve{w}_{t-1}\right)^\top \ve{x}_t$, and $r_t = \ve{u}^\top \ve{x}_t - y_t$,
so that $\Delta = \eta_t \cdot (s_t - r_t) \cdot \ve{x}_t$ and $R(\ve{w}_{1 : T} | \ve{u} ) = \sum_{t = 1}^T \{ s_t^2 - r_t^2 \}$.
We have
\begin{align*}
  D_{\varphi}\left( \ve{u} \left\| \ve{w}_{t-1}\right.\right) - D_{\varphi}\left( \ve{u} \left\| \ve{w}_{t}\right. \right) &\geq \eta_t \cdot (s_t - r_t) \cdot s_t - \eta_t^2 \cdot (s_t - r_t)^2 \cdot \frac{p - 1}{2} \cdot \| \ve{x} \|_p^2 \\
  &= \eta_t \cdot (s_t^2 - s_t \cdot r_t) - \eta_t^2 \cdot (s_t - r_t)^2 \cdot \frac{p - 1}{2} \cdot \| \ve{x} \|_p^2 \\
  &= \frac{1}{2} \eta_t \cdot (s_t^2 - r_t^2) + \frac{1}{2} \eta_t \cdot (s_t - r_t)^2 \cdot \left( 1 - \eta_t \cdot (p - 1) \cdot \| \ve{x} \|_p^2 \right) \\
  &\geq \frac{1}{2} \eta_t \cdot (s_t^2 - r_t^2) + \frac{1}{2} \eta_t \cdot (s_t - r_t)^2 \cdot \left( 1 - \eta_t \cdot (p - 1) \cdot X_p^2 \right).
\end{align*}
We now fix
\begin{eqnarray}
\eta_t & = & \frac{1}{(p - 1) \cdot X_p^2} \:\:,\label{defeta}
\end{eqnarray}
so that the last term disappears.
We finally get:
$$ (1/2) \| \ve{u} \|_q^2 \geq \frac{1}{2} \cdot \eta_t \cdot R(\ve{w}_{1:T} | \ve{u}), $$
so that
\begin{eqnarray}
R(\ve{w}_{1:T} | \ve{u}) & \leq & \frac{\| \ve{u} \|_q^2}{\eta_t} \nonumber \\
& = & (p - 1) \cdot X_p^2 \cdot \| \ve{u} \|_q^2 \nonumber.
\end{eqnarray}
as claimed.

One can also derive a bound for the prediction regret, commonly studied in online learning.
This is because if we modify choice of $\eta_t$ to $\frac{\alpha}{1 + \alpha} \cdot \frac{1}{(p - 1) \cdot X_p^2}$, Equation \ref{eqn:kivinen-bound} can be further bounded as
\begin{align*}
 	D_{\varphi}\left(\ve{u} \left\| \ve{w}_{t-1}\right.\right) - D_{\varphi}\left(\ve{u} \left\| \ve{w}_{t}\right.\right) &\geq \eta_t \cdot (y_t - \ve{w}_{t-1}^\top \ve{x}_t) \cdot \left(\ve{u} - \ve{w}_{t-1}\right)^\top \ve{x}_t - \frac{1}{2} \cdot \frac{\alpha}{1 + \alpha} \cdot \eta_t \cdot \frac{1}{X_p^2} \cdot (y_t - \ve{w}_{t-1}^\top \ve{x}_t)^2 \cdot \| \ve{x} \|_p^2 \\
 	&\geq \eta_t \cdot (y_t - \ve{w}_{t-1}^\top \ve{x}_t) \cdot \left(\ve{u} - \ve{w}_{t-1}\right)^\top \ve{x}_t - \frac{1}{2} \cdot \frac{\alpha}{1 + \alpha} \cdot \eta_t \cdot (y_t - \ve{w}_{t-1}^\top \ve{x}_t)^2 \\
 	&\geq \frac{1}{2} \cdot \eta_t \cdot (y_t - \ve{w}_{t - 1}^\top \ve{x}_t)^2 - (1 + \alpha) \cdot \frac{1}{2} \cdot \eta_t \cdot (y_t - \ve{u}^\top \ve{x}_t)^2,
\end{align*}
where the last inequality is a simple completing the square argument \citep[Lemma 5.1]{kwEG}.
This gives a prediction regret bound of \citep{glTR}
$$ \frac{1}{2} \sum_{t = 1}^T (y_t - \ve{w}_{t-1}^\top \ve{x}_t)^2 - \frac{1}{2} \cdot \sum_{t = 1}^T (y_t - \ve{u}^\top \ve{x}_t)^2 \leq \frac{\alpha}{2} \cdot \sum_{t = 1}^T (y_t - \ve{u}^\top \ve{x}_t)^2 + \frac{1 + \alpha}{\alpha} \cdot \frac{p - 1}{2} \cdot X_p^2 \| \ve{u} \|_q^2. $$


\newpage

%
\subsection{Corrected regret analysis}

Let $\varphi_q^\dagger( \ve{x} ) = \| \ve{x} \|_q$.
It may be checked that for any $\ve{x}$,
$$ \nabla \varphi_p^\dagger( \nabla \varphi_q^\dagger( \ve{x} ) ) = \frac{\ve{x}}{\| \ve{x} \|_q}. $$
Also, for any $\ve{x}$,
$$ \| \nabla \varphi_p^\dagger( \ve{x} ) \|_q = 1. $$
Note that the corresponding $\varphi( \ve{x} ) = (1/2) \| \ve{x} \|_q^2$, with $g(\ve{x}) = \| \ve{x} \|_q$.

We have $\ve{w}_{t} = \nabla \varphi_p^\dagger( \ve{\theta}_t )$, where
$\ve{\theta}_t = \nabla \varphi_q^\dagger( \ve{w}_{t - 1} ) - \Delta_t$ for
$\Delta_t = \eta_t \cdot ( \ve{w}_{t - 1}^\top \ve{x}_t - y_t )$.
Note then that
$$ \| \ve{w}_t \|_q = \| \nabla \varphi_p^\dagger( \ve{\theta}_t ) \|_q = 1. $$


\emph{Step 1: Telescoping sum}.
We have
\begin{eqnarray}
D_{\varphi^\dagger}(\ve{u}\| \ve{w}_0) & \geq & D_{\varphi^\dagger}(\ve{u}\| \ve{w}_0) - D_{\varphi^\dagger}(\ve{u}\| \ve{w}_{T+1}) \nonumber\\
  & = & \sum_{t=1}^T  \left\{D_{\varphi^\dagger}(\ve{u}\| \ve{w}_{t-1}) - D_{\varphi^\dagger}(\ve{u}\| \ve{w}_{t})\right\} \nonumber \text{ by telescoping property }.
\end{eqnarray}


\emph{Step 1.5: Bregman gauge lemma}.
Applying Theorem \ref{th00},
\begin{align*}
 	D_{\varphi^\dagger}(\ve{u}\| \ve{w}_0) &\geq \sum_{t=1}^T  \left\{D_{\varphi^\dagger}(\ve{u}\| \ve{w}_{t-1}) - D_{\varphi^\dagger}(\ve{u}\| \ve{w}_{t})\right\} \\
 	&\geq \| u \|_q \cdot \sum_{t=1}^T  \left\{ D_{\varphi}\left( \frac{\ve{u}}{\| \ve{u} \|_q} \| \ve{w}_{t-1} \right) - D_{\varphi}\left( \frac{\ve{u}}{\| \ve{u} \|_q} \| \ve{w}_{t} \right) \right\}.
 \end{align*}


\emph{Step 2: Bregman triangle equality}.
The Bregman triangle equality brings:
\begin{eqnarray}
D_{\varphi}\left( \frac{\ve{u}}{\| \ve{u} \|_q} \| \ve{w}_{t-1} \right) - D_{\varphi}\left( \frac{\ve{u}}{\| \ve{u} \|_q} \| \ve{w}_{t} \right) \nonumber & = & \left( \frac{\ve{u}}{\| \ve{u} \|_q} - \ve{w}_{t-1}\right)^\top \left(\nabla\varphi\left( \ve{w}_{t}\right)-\nabla\varphi\left( \ve{w}_{t-1}\right)\right) - D_{\varphi}\left(  \ve{w}_{t-1}\left\| \ve{w}_{t}\right.\right) \nonumber.
\end{eqnarray}


\emph{Step 3: Simplification of divergence term}.
Since $\| \ve{w}_t \|_q = 1$, applying Theorem \ref{th00} again,
\begin{align*}
	D_{\varphi}\left(  \ve{w}_{t-1} \left\| \ve{w}_{t}\right.\right) &= D_{\varphi^\dagger}\left( \ve{w}_{t-1} \left\| \ve{w}_{t} \right.\right) \\
	&= \varphi^\dagger( \ve{w}_{t-1} ) - \varphi^\dagger( \ve{w}_{t} ) - \nabla\varphi^\dagger( \ve{w}_{t} )^\top ( \ve{w}_{t-1} - \ve{w}_{t} ) \\
	&= -\nabla\varphi^\dagger( \ve{w}_{t} )^\top ( \ve{w}_{t-1} - \ve{w}_{t} ) \\
	&= \varphi^\dagger( \ve{w}_{t} ) - \nabla\varphi^\dagger( \ve{w}_{t} )^\top \ve{w}_{t - 1} \text{ by norm homogeneity. } \\
	&= 1 - \nabla\varphi^\dagger( \ve{w}_{t} )^\top \ve{w}_{t - 1}.
\end{align*}
Note also that
$$ \nabla\varphi( \ve{w}_t ) = \nabla\varphi^\dagger( \ve{w}_t ). $$
Thus,
\begin{align*}
 	\ve{w}_{t - 1}^\top \left(\nabla\varphi\left( \ve{w}_{t}\right)-\nabla\varphi\left( \ve{w}_{t-1}\right)\right) &= \ve{w}_{t - 1}^\top \left(\nabla\varphi^\dagger\left( \ve{w}_{t}\right)-\nabla\varphi^\dagger\left( \ve{w}_{t-1}\right)\right) \\
 	&= \ve{w}_{t - 1}^\top \nabla\varphi^\dagger\left( \ve{w}_{t}\right) - \varphi^\dagger\left( \ve{w}_{t-1}\right) \\
 	&= \ve{w}_{t - 1}^\top \nabla\varphi^\dagger\left( \ve{w}_{t}\right) - 1 \\
 	&= -D_{\varphi}\left(  \ve{w}_{t-1} \left\| \ve{w}_{t}\right.\right).
 \end{align*}
So,
$$ D_{\varphi}\left( \frac{\ve{u}}{\| \ve{u} \|_q} \| \ve{w}_{t-1} \right) - D_{\varphi}\left( \frac{\ve{u}}{\| \ve{u} \|_q} \| \ve{w}_{t} \right) = \left( \frac{\ve{u}}{\| \ve{u} \|_q} \right)^\top \left( \nabla\varphi\left( \ve{w}_{t}\right)-\nabla\varphi\left( \ve{w}_{t-1}\right) \right). $$


\emph{Step 3.5: Simplification of difference term}.
We have
\begin{align*}
	\nabla\varphi\left( \ve{w}_{t}\right) - \nabla\varphi\left( \ve{w}_{t-1}\right) &= \nabla\varphi_q^\dagger\left( \ve{w}_{t}\right) - \nabla\varphi_q^\dagger\left( \ve{w}_{t-1}\right) \\
	&= \nabla\varphi_q^\dagger\left( \nabla\varphi_p^\dagger( \ve{\theta}_t ) \right) - \nabla\varphi_q^\dagger\left( \ve{w}_{t-1}\right) \\
	&= \frac{\ve{\theta}_t}{\| \ve{\theta}_t \|_p} - \nabla\varphi_q^\dagger\left( \ve{w}_{t-1}\right) \\
	&= \frac{\ve{\theta}_t}{\| \ve{\theta}_t \|_p} - \ve{\theta}_t - \Delta_t \\
	&= \frac{(1 - \| \ve{\theta}_t \|_p) \cdot \ve{\theta}_t - \| \ve{\theta}_t \|_p \cdot \Delta_t}{\| \ve{\theta}_t \|_p}.
\end{align*}
So,
$$ D_{\varphi}\left( \frac{\ve{u}}{\| \ve{u} \|_q} \| \ve{w}_{t-1} \right) - D_{\varphi} \left( \frac{\ve{u}}{\| \ve{u} \|_q} \| \ve{w}_{t} \right) = \frac{(1 - \| \ve{\theta}_t \|_p)}{\| \ve{\theta}_t \|_p} \cdot \left( \frac{\ve{u}}{\| \ve{u} \|_q} \right)^\top \ve{\theta}_t - \left( \frac{\ve{u}}{\| \ve{u} \|_q} \right)^\top \Delta_t, $$
We end up with
$$ D_{\varphi^\dagger}(\ve{u}\| \ve{w}_0) \geq \sum_{t = 1}^T \left\{ \frac{(1 - \| \ve{\theta}_t \|_p)}{\| \ve{\theta}_t \|_p} \cdot \ve{u}^\top \ve{\theta}_t - \ve{u}^\top \Delta_t \right\}. $$


\emph{Step 4: Simplification and choice of $\eta$}.
Note that

\scalebox{0.9}{
\begin{minipage}{\linewidth}
\begin{align*}
	-\ve{u}^\top \Delta_t &= \eta_t \cdot (\ve{u}^\top \ve{x}_t) \cdot (y_t - \ve{w}_{t-1}^\top \ve{x}_t) \\
	&= \eta_t \cdot (\ve{u}^\top \ve{x}_t - y_t + y_t) \cdot (y_t - \ve{w}_{t-1}^\top \ve{x}_t) \\
	&= \eta_t \cdot (\ve{u}^\top \ve{x}_t - y_t) \cdot (y_t - \ve{w}_{t-1}^\top \ve{x}_t) + \eta_t \cdot y_t \cdot (y_t - \ve{w}_{t-1}^\top \ve{x}_t) \\
	&= -\eta_t \cdot (\ve{u}^\top \ve{x}_t - y_t) \cdot (\ve{w}_{t-1}^\top \ve{x}_t - y_t) + \eta_t \cdot y_t \cdot (y_t - \ve{w}_{t-1}^\top \ve{x}_t) \\
	&= (1/2) \cdot \eta_t \cdot ( (\ve{u}^\top \ve{x}_t - \ve{w}_{t-1}^\top \ve{x}_t)^2 - (\ve{u}^\top \ve{x}_t - y_t)^2 - (\ve{w}_{t-1}^\top \ve{x}_t - y_t)^2 ) + \eta_t \cdot y_t \cdot (y_t - \ve{w}_{t-1}^\top \ve{x}_t) \\
	&= (1/2) \cdot \eta_t \cdot ( (\ve{u}^\top \ve{x}_t - \ve{w}_{t-1}^\top \ve{x}_t)^2 - (\ve{u}^\top \ve{x}_t - y_t)^2 ) - (1/2) \cdot \eta_t \cdot ( (\ve{w}_{t-1}^\top \ve{x}_t - y_t)^2 - 2 \cdot y_t \cdot (y_t - \ve{w}_{t-1}^\top \ve{x}_t) ) \\
	&= (1/2) \cdot \eta_t \cdot ( (\ve{u}^\top \ve{x}_t - \ve{w}_{t-1}^\top \ve{x}_t)^2 - (\ve{u}^\top \ve{x}_t - y_t)^2 ) - (1/2) \cdot \eta_t \cdot ( (\ve{w}_{t-1}^\top \ve{x}_t)^2 - y_t^2 ).
	%&\geq (1/2) \cdot \eta_t \cdot ( (\ve{u}^\top \ve{x} - \ve{w}_{t-1}^\top \ve{x}_t)^2 - (\ve{u}^\top \ve{x} - y_t)^2 ) - (1/2) \cdot \eta_t \cdot (\ve{w}_{t-1}^\top \ve{x}_t)^2 \\
	%&\geq (1/2) \cdot \eta_t \cdot ( (\ve{u}^\top \ve{x} - \ve{w}_{t-1}^\top \ve{x}_t)^2 - (\ve{u}^\top \ve{x} - y_t)^2 ) - (1/2) \cdot \eta_t \cdot W_q^2 X_p^2.
\end{align*}
\end{minipage}
}

So,
\begin{align*}
 	D_{\varphi^\dagger}(\ve{u}\| \ve{w}_0) &\geq \sum_{t = 1}^T \left\{ \frac{(1 - \| \ve{\theta}_t \|_p)}{\| \ve{\theta}_t \|_p} \cdot \ve{u}^\top \ve{\theta}_t \right\} + (1/2) \cdot \eta_t \cdot \sum_{t = 1}^T ( (\ve{u}^\top \ve{x} - \ve{w}_{t-1}^\top \ve{x}_t)^2 - (\ve{u}^\top \ve{x} - y_t)^2 ) - ( (\ve{w}_{t-1}^\top \ve{x}_t)^2 - y_t^2 ) \\
 	&\geq \sum_{t = 1}^T \left\{ \frac{(1 - \| \ve{\theta}_t \|_p)}{\| \ve{\theta}_t \|_p} \cdot \ve{u}^\top \ve{\theta}_t \right\} + (1/2) \cdot \eta_t \cdot R( \ve{w}; \ve{u} ) - (1/2) \cdot \eta_t \cdot \sum_{t = 1}^T ( (\ve{w}_{t-1}^\top \ve{x}_t)^2 - y_t^2 ) \\
\end{align*}


%
% \subsection{A questionable proof}

% %
% \begin{proof}[Questionable Proof of Lemma \ref{lemlplq}]
% We proceed \textit{e.g.} as in \citet{kwhTP}.
% We first note that
% $D_{\varphi^\dagger}(\ve{u}\| \ve{w}_0) = W_q\cdot \|\ve{u}\|_q$ since $\ve{w}_0 = \ve{0}$, and $D_{\varphi^\dagger}(\ve{u}\| \ve{w}_{T+1}) \geq 0$, and so

% %\resizebox{0.9\linewidth}{!}{
% \begin{minipage}{\linewidth}
% \begin{eqnarray}
% W_q\cdot\|\ve{u}\|_q & \geq & D_{\varphi^\dagger}(\ve{u}\| \ve{w}_0) - D_{\varphi^\dagger}(\ve{u}\| \ve{w}_{T+1}) \nonumber\\
%   & = & \sum_{t=1}^T  \left\{ D_{\varphi^\dagger}(\ve{u}\| \ve{w}_{t-1}) - D_{\varphi^\dagger}(\ve{u}\| \ve{w}_{t}) \right\}\nonumber \text{ by telescoping property }.
% \end{eqnarray}
% \end{minipage}
% %}

% The Bregman triangle equality (also called the three points property) \citep[Property 5]{bnnBV}, \citep[Lemma 11.1]{Cesa-Bianchi:2006} brings:
% \begin{eqnarray}
% \label{eqn:bregman-3pp}
% D_{\varphi^\dagger}(\ve{u}\| \ve{w}_{t-1}) - D_{\varphi^\dagger}(\ve{u}\| \ve{w}_{t}) & = & \left(\ve{u} - \ve{w}_{t-1}\right)^\top \left(\nabla\varphi^\dagger\left( \ve{w}_{t}\right)-\nabla\varphi^\dagger\left( \ve{w}_{t-1}\right)\right) - D_{\varphi^\dagger}\left(  \ve{w}_{t-1}\left\| \ve{w}_{t}\right.\right).
% \end{eqnarray}
% The last divergence term can be bounded by invoking Corollary
% \ref{corr:update-bound}, which gives:
% \begin{eqnarray}
% D_{\varphi^\dagger}\left(\ve{w}_{t-1} \| \ve{w}_t \right) & \leq & \frac{p-1}{2} \cdot \frac{W_q \upeta_t^2 X_p^2}{W_q - \eta_t (X_p+W_qX^2_p)}\:\:.\label{bDP}
% \end{eqnarray}
% As per \citet{kwhTP}, let $s_t = \left( \ve{u} - \ve{w}_{t-1}\right)^\top \ve{x}_t$, and $r_t = \ve{u}^\top \ve{x}_t - y_t$,
% so that $\upeta_t = \eta_t \cdot (s_t - r_t)$ and $R(\ve{w}_{1 : T} | \ve{u} ) = \sum_{t = 1}^T \{ s_t^2 - r_t^2 \}$.
% We have
% \begin{align*}
% D_{\varphi^\dagger}(\ve{u}\| \ve{w}_{t-1}) - D_{\varphi^\dagger}(\ve{u}\| \ve{w}_{t}) &\geq \eta_t \cdot (s_t - r_t) \cdot s_t - \eta_t^2 \cdot (s_t - r_t)^2 \cdot \frac{p - 1}{2} \cdot \frac{W_q X_p^2}{W_q - \eta_t (X_p+W_qX^2_p)} \\
%   &= \eta_t \cdot (s_t^2 - s_t \cdot r_t) - \eta_t^2 \cdot (s_t - r_t)^2 \cdot \frac{p - 1}{2} \cdot \frac{W_q X_p^2}{W_q - \eta_t (X_p+W_qX^2_p)} \\
%   &= \frac{1}{2} \eta_t \cdot (s_t^2 - r_t^2) + \frac{1}{2} \eta_t \cdot (s_t - r_t)^2 \cdot \left( 1 - \eta_t \cdot (p - 1) \cdot \frac{W_q X_p^2}{W_q - \eta_t (X_p+W_qX^2_p)} \right).
% \end{align*}
% We now fix
% \begin{eqnarray}
% \eta_t & = & \frac{W_q}{X_p+p W_q X_p^2}\:\:,\label{defeta}
% \end{eqnarray}
% so that the last term disappears.
% We check that since $p\geq 1$, we indeed have $\eta_t \leq W_q/(X_p + W_q X_p^2)$, so that Corollary \ref{corr:update-bound}) is applicable.
% We finally get:
% \begin{eqnarray}
% \sum_{t=1}^T D_{\varphi^\dagger}\left( \ve{u}\left\|   \ve{w}_{t-1}\right.\right) - D_{\varphi^\dagger}\left( \ve{u}\left\| \ve{w}_{t}\right.\right)  & \geq &  \frac{1}{2} \cdot \eta_t \cdot R(\ve{w}_{1:T} | \ve{u}) \:\:.
% \end{eqnarray}
% We then combine with Equation (\ref{eq111}), use the fact that $g_{q}(\ve{u}) = \|\ve{u}\|_q / W_q$, and get
% \begin{eqnarray}
% R(\ve{w}_{1:T} | \ve{u}) & \leq & \frac{2}{\eta_t} \cdot {W_q \cdot \| \ve{u} \|_q} \nonumber \\
% & = & 2 \| \ve{u} \|_q X_p (1+p W_q X_p) \nonumber \:\:,
% \end{eqnarray}
% as claimed.
% \end{proof}

% We can contrast Equation \ref{eqn:bregman-3pp} with Equation \ref{eq111}.
% Essentially, the two are identical because we have
% \begin{align*}
% 	D_{\varphi^\dagger}( \ve{w}_{t-1} \| \ve{w}_{t} ) &= \varphi^\dagger( \ve{w}_{t-1} ) - \nabla\varphi^\dagger( \ve{w}_{t} )^\top \ve{w}_{t-1} \text{ by Corollary 6 [HARD LINK] }  \\
% 	&= \nabla\varphi^\dagger( \ve{w}_{t-1} )^\top \ve{w}_{t-1} - \nabla\varphi^\dagger( \ve{w}_{t} )^\top \ve{w}_{t-1} \text{ since } \varphi \text{ is a norm, and hence 1-homogenous }  \\
% 	&= ( \nabla\varphi^\dagger( \ve{w}_{t-1} ) - \nabla\varphi^\dagger( \ve{w}_{t} ) )^\top \ve{w}_{t-1},
% \end{align*}
% so that a scaling by $g(\ve{u})$ is effectively compensated for.
% Note that this also implies
% $$ D_{\varphi^\dagger}(\ve{u}\| \ve{w}_{t-1}) - D_{\varphi^\dagger}(\ve{u}\| \ve{w}_{t}) = \eta_t \cdot (\ve{u}^\top \ve{x}) \cdot (y_t - \ve{w}_{t-1}^\top \ve{x}_t). $$
% It is of interest whether such an identity may be useful.
% Going down this route, we apparently would not even need an explicit bound on the divergence between subsequent iterates.
% Note that

% \scalebox{0.825}{
% \begin{minipage}{\linewidth}
% \begin{align*}
% 	\eta_t \cdot (\ve{u}^\top \ve{x}) \cdot (y_t - \ve{w}_{t-1}^\top \ve{x}_t) &= \eta_t \cdot (\ve{u}^\top \ve{x} - y_t + y_t) \cdot (y_t - \ve{w}_{t-1}^\top \ve{x}_t) \\
% 	&= \eta_t \cdot (\ve{u}^\top \ve{x} - y_t) \cdot (y_t - \ve{w}_{t-1}^\top \ve{x}_t) + \eta_t \cdot y_t \cdot (y_t - \ve{w}_{t-1}^\top \ve{x}_t) \\
% 	&= -\eta_t \cdot (\ve{u}^\top \ve{x} - y_t) \cdot (\ve{w}_{t-1}^\top \ve{x}_t - y_t) + \eta_t \cdot y_t \cdot (y_t - \ve{w}_{t-1}^\top \ve{x}_t) \\
% 	&= (1/2) \cdot \eta_t \cdot ( (\ve{u}^\top \ve{x} - \ve{w}_{t-1}^\top \ve{x}_t)^2 - (\ve{u}^\top \ve{x} - y_t)^2 - (\ve{w}_{t-1}^\top \ve{x}_t - y_t)^2 ) + \eta_t \cdot y_t \cdot (y_t - \ve{w}_{t-1}^\top \ve{x}_t) \\
% 	&= (1/2) \cdot \eta_t \cdot ( (\ve{u}^\top \ve{x} - \ve{w}_{t-1}^\top \ve{x}_t)^2 - (\ve{u}^\top \ve{x} - y_t)^2 ) - (1/2) \cdot \eta_t \cdot ( (\ve{w}_{t-1}^\top \ve{x}_t - y_t)^2 - 2 \cdot y_t \cdot (y_t - \ve{w}_{t-1}^\top \ve{x}_t) ) \\
% 	&= (1/2) \cdot \eta_t \cdot ( (\ve{u}^\top \ve{x} - \ve{w}_{t-1}^\top \ve{x}_t)^2 - (\ve{u}^\top \ve{x} - y_t)^2 ) - (1/2) \cdot \eta_t \cdot ( (\ve{w}_{t-1}^\top \ve{x}_t)^2 - y_t^2 ) \\
% 	&\geq (1/2) \cdot \eta_t \cdot ( (\ve{u}^\top \ve{x} - \ve{w}_{t-1}^\top \ve{x}_t)^2 - (\ve{u}^\top \ve{x} - y_t)^2 ) - (1/2) \cdot \eta_t \cdot (\ve{w}_{t-1}^\top \ve{x}_t)^2 \\
% 	&\geq (1/2) \cdot \eta_t \cdot ( (\ve{u}^\top \ve{x} - \ve{w}_{t-1}^\top \ve{x}_t)^2 - (\ve{u}^\top \ve{x} - y_t)^2 ) - (1/2) \cdot \eta_t \cdot W_q^2 X_p^2.
% \end{align*}
% \end{minipage}
% }
% We conclude that
% \begin{align*}
% 	\sum_{t = 1}^T (1/2) \cdot \eta_t \cdot  ( (\ve{u}^\top \ve{x} - \ve{w}_{t-1}^\top \ve{x}_t)^2 - (\ve{u}^\top \ve{x} - y_t)^2 ) &\leq W_q \cdot \| \ve{u} \|_q + W_q^2 X_p^2 \cdot \sum_{t = 1}^T (1/2) \cdot \eta_t.
% \end{align*}
% For a constant learning rate $\eta_t \equiv \eta$,
% $$ R(\ve{w}_{1:T} | \ve{u}) \leq \frac{2 \cdot W_q \cdot \| \ve{u} \|_q}{\eta} + T \cdot W_q^2 X_p^2. $$
% This seems to suggest choosing $\eta$ large is a good idea, which is a dubious claim.

